Graph-Theoretic Bounds for Non-Linear Function Computation Broadcast

This work studies non-linear function computation broadcast (NFCB), in which a sender with access to $N$ datasets $(X_1,\dots,X_N)$ broadcasts a common message to $K$ users, each possessing side information and requesting a function of the datasets. The goal is to minimize the rate required for asymptotically lossless recovery of all demands. We introduce a broadcast graph that jointly captures the source distribution, side information, and demanded functions. Using K\"orner's characteristic-graph framework, we develop an achievable scheme for arbitrary $K$, general source distributions, and general finite-field demands, including linear, non-separable, and non-linear functions, without restricting the encoding or decoding operations to be linear. We also present a side-information-assisted independent-set scheme and characterize the optimal graph-based achievable rate for compatible functions. For the converse, we derive a multi-letter response-profile bound that strengthens a basic side-information converse, zero-error and asymptotically lossless clique-entropy bounds based on the operational block broadcast graph, and a genie-aided lower bound. For binary NFCB with $N=K$ and side information $X_i$ at user $i$, we characterize the optimal rate in several special cases and bound the worst-case and average additive gaps between the proposed achievable rate and the genie-aided converse for $K=3$ and $K=4$. Finally, three-user examples with Boolean and linear demands illustrate the proposed bounds and show that non-linear encoding can strictly outperform the best scalar and vector linear schemes.

==> plots/4user_graph_text.tex <==

\foreach \pos/\name/\value/\colo/\labelpos in {
% {(0,0.6)/a/0000/black!30!white/above}, 
% {(0.38,0.52)/b/0001/black!30!white/above}, 
% {(0.70,0.30)/c/0010/black!30!white/above}, 
% {(0.92,-0.08)/d/0011/black!30!white/above}, 
% {(0.92,-0.38)/e/0100/black!30!white/below}, 
% {(0.7,-0.7)/f/0101/black!30!white/below},
% {(0.38,-0.92)/g/0110/black!30!white/below},
% {(0,-1)/h/0111/black!30!white/below},
% {(-0.5,-1)/i/1000/black!30!white/below},
% {(-0.88,-0.92)/j/1001/black!30!white/below},
% {(-1.2,-0.7)/k/1010/black!30!white/below},
% {(-1.42,-0.38)/l/1011/black!30!white/below},
% {(-1.42,-0.08)/m/1100/black!30!white/above},
% {(-1.20,0.30)/n/1101/black!30!white/above},
% {(-0.88,0.52)/o/1110/black!30!white/above},
% {(-0.5,0.6)/p/1111/black!30!white/above}}
{(0,0.65)/a/0000/black!30!white/above}, 
{(0.43,0.52)/b/0001/black!30!white/above}, 
{(0.70,0.30)/c/0010/black!30!white/above}, 
{(0.87,-0.08)/d/0011/black!30!white/above}, 
{(0.87,-0.38)/e/0100/black!30!white/below}, 
{(0.7,-0.7)/f/0101/black!30!white/below},
{(0.43,-0.92)/g/0110/black!30!white/below},
{(0,-1.05)/h/0111/black!30!white/below},
{(-0.5,-1.05)/i/1000/black!30!white/below},
{(-0.93,-0.92)/j/1001/black!30!white/below},
{(-1.15,-0.7)/k/1010/black!30!white/below},
{(-1.37,-0.38)/l/1011/black!30!white/below},
{(-1.37,-0.08)/m/1100/black!30!white/above},
{(-1.15,0.30)/n/1101/black!30!white/above},
{(-0.93,0.52)/o/1110/black!30!white/above},
{(-0.5,0.65)/p/1111/black!30!white/above}}
            \node[draw, circle, inner sep=2pt, fill=black, label={[label distance=1mm]\labelpos:$\value$}](\name) at \pos {};


==> plots/figtext.tex <==
\foreach \pos/\name/\value/\colo/\labelpos in {{(2,3)/a/000/black!30!white/above}, {(3,2)/b/001/black!30!white/above}, {(3,1)/c/010/black!30!white/below}, {(2,0)/d/011/black!30!white/below}, {(1,0)/e/100/black!30!white/below}, {(0,1)/f/101/black!30!white/below},{(0,2)/g/110/black!30!white/above},{(1,3)/h/111/black!30!white/above}}
            \node[draw, circle, inner sep=2pt, fill=black, label={[label distance=1mm]\labelpos:$\value$}](\name) at \pos {};
